InstructMol: Multi-Modal Integration for Building a Versatile and Reliable Molecular Assistant in Drug Discovery

The rapid evolution of artificial intelligence in drug discovery encounters challenges with generalization and extensive training, yet Large Language Models (LLMs) offer promise in reshaping interactions with complex molecular data. Our novel contribution, InstructMol, a multi-modal LLM, effectively aligns molecular structures with natural language via an instruction-tuning approach, utilizing a two-stage training strategy that adeptly combines limited domain-specific data with molecular and textual information. InstructMol showcases substantial performance improvements in drug discovery-related molecular tasks, surpassing leading LLMs and significantly reducing the gap with specialized models, thereby establishing a robust foundation for a versatile and dependable drug discovery assistant.

==> sec/X_suppl_arxiv.tex <==
% \setcounter{page}{1}
% \maketitlesupplementary

\noindent
This supplementary material includes additional details and results not included in the main paper due to page limitations. The items included are as follows:

\begin{itemize}[leftmargin=*]
    \item Elaboration on task definitions and datasets in Sec \ref{appendix:task-def}.
    \item Implementation details about training in Sec \ref{sec:implementation_details}.
    \item Further details regarding evaluation metrics in Sec \ref{appendix:eval-metric}.
    \item Illustrative samples of instructions for each task (refer to Tab \ref{tab:appendix-dataset}) and examples of the process for constructing prompts in the context of few-shot in-context learning (refer to Fig \ref{tab:appendix-ICL-prompt}).
    \item Additional results for each task and several challenging cases in Sec. \ref{appendix:more-examples}.
    \item Comparison with Agent-based systems in Sec. \ref{appendix:Comparison_with_agents}.
\end{itemize}



\section{Tasks Definition and Dataset Details}
\label{appendix:task-def}

\begin{table}[ht]
\small
\vskip -0.07in
\centering
\setlength{\tabcolsep}{6mm}{
\scalebox{0.8}{
\begin{tabular}{lcc}
    \toprule
    \textsc{tasks} & \textsc{\# Samples} & \textsc{Data Source} \\
    \midrule
    Alignment Pretrain & 264K & PubMed~\cite{PubChem} \\
    Property Prediction(Regression) & 362K & QM9~\cite{Mol-Instructions, MoleculeNet} \\ 
    Property Prediction(Classification) &35,742 & BACE, BBBP, HIV~\cite{MoleculeNet} \\
    Molecule Description Generation & 26,507 & ChEBI-20~\cite{Text2Mol} \\
    Forward Prediction & 125K & USPTO~\cite{Mol-Instructions, USPTO} \\ 
    Retrosynthesis & 130K & USPTO\_500MT~\cite{Mol-Instructions, USPTO_500MT} \\ 
    Reagent Prediction & 125K & USPTO\_500K~\cite{Mol-Instructions, USPTO_500MT} \\
    \bottomrule
    
\end{tabular}
}}
\caption{\footnotesize
Details of InstrutMol two-stage training data.
}
\vskip -0.1in
\label{tab:data_collection}
\end{table}


\paragraph{Property Prediction.}
Molecular Property Prediction involves the forecasting or estimation of the biophysical and chemical properties of a molecule. 
% This methodology expedites the evaluation of a wide spectrum of molecular properties, facilitating the virtual screening of compounds. Furthermore, it enables the anticipation of unknown characteristics in novel molecules, thus enhancing research efficacy and minimizing developmental timelines. 
In this work, our emphasis lies on three binary classification tasks sourced from the MoleculeNet benchmark (BBBP, BACE, and HIV)~\cite{MoleculeNet}, and three regression tasks concentrating on the quantum properties of molecules from the QM9~\cite{QM9} dataset.


\paragraph{Molecule Description Generation.}
Generating molecular descriptions involves compiling a detailed overview of a molecule's structure, properties, activities, and functions. This process aids chemists and biologists by swiftly providing crucial molecular insights for their research. Our data collection involves the extraction of molecular text annotations from PubChem~\cite{PubChem}. Leveraging PubChem's \textbf{Power User Gateway}~\cite{PUG-View}, we retrieve abstracts of compound records in XML format. Subsequently, we extracted valid molecular description texts identified by unique PubChem Chemical Identifiers (CIDs), filtering out SMILES strings with syntactic errors or deviations from established chemical principles. Furthermore, we utilize the ChEBI-20 dataset~\cite{Text2Mol} for downstream tasks in molecule description generation, comprising 33,010 molecule description pairs divided into 80\% for training, 10\% for validation and 10\% for testing. To prevent data leakage, compounds in the PubChem text annotations that coincide with the ChEBI-20 test split are excluded.


\paragraph{Forward Reaction Prediction.}
Predicting the forward reaction involves anticipating the probable product(s) of a chemical reaction based on given reactants and reagents. 
% This process streamlines research optimization, reduces experimental guesswork, and promotes eco-friendly chemistry by minimizing waste. 
For this task, we utilize the forward-reaction-prediction dataset from \cite{Mol-Instructions}, comprising 138,768 samples sourced from the USPTO dataset~\cite{USPTO}. Each entry includes reactants and reagents separated by '.' within the instruction and with the output product.

\paragraph{Reagent Prediction.}
Reagent prediction identifies the substances necessary for a chemical reaction, helping to discover new types of reactions and optimal conditions. We use the reagent Prediction data from~\cite{Mol-Instructions}, sourced from the USPTO\_500MT dataset~\cite{USPTO_500MT}. Each entry features a chemical reaction indicated as ``reactants $>>$ product", with the output indicating the reagents involved in the reaction.

\paragraph{Retrosynthesis Prediction.}
Retrosynthetic analysis in organic chemistry reverses engineering by tracing potential synthesis routes from the target compound backward. This strategy is vital for efficient synthesis of complex molecules and for fostering innovation in pharmaceuticals and materials. For this task, we also used the dataset from \cite{Mol-Instructions}, which is sourced from USPTO\_500MT. The data organize inputs as products and outputs as reactants separated by '.' for each compound.


\section{Implementation Details}
\label{sec:implementation_details}

\textbf{Model Settings.}
A graph neural network with five graph isomorphism network (GIN)~\cite{GIN} layers is used as the molecule graph encoder $f_g$. The hidden dimension is set to be 300. The GIN model is initialized using the MoleculeSTM~\cite{moleculeSTM} graph encoder, which is pre-trained through molecular graph-text contrastive learning. We employ Vicuna-v-1.3-7B~\cite{vicuna} as the base LLM, which has been trained through instruction-tuning. The total number of parameters of InstructMol is around 6.9B. 

\noindent
\textbf{Training Details.} In the first stage, we employ the training split comprising around 264K molecule-caption pairs from PubMed. Using a batch size of 128, we conduct training for 5 epochs. We use the AdamW optimizer, with $\beta$=(0.9, 0.999) and a learning rate of 2e-3, without weight decay. Warm-up is executed over 3\% of the total training steps, followed by a cosine schedule for learning rate decay. 
% To enhance processing efficiency, we convert a sparse batch of graphs into a dense batch. 
For the second stage, we conduct training for three specific scenarios. For fair comparisons with traditional methods, training spans 20 to 50 epochs for the molecule description generation task using the ChEBI-20 training split. Property prediction and reaction tasks undergo 10 epochs using corresponding instruction datasets. In InstructMol training, we maintain a consistent batch size of 128 and set the learning rate to 8e-5. Linear layers within the LLM utilize a LoRA rank of 64 and a scaling value $\alpha$ of 16. All experiments are run with 4$\times$RTX A6000 (48GB) GPUs.


\begin{table}[h]
\small
\centering
\renewcommand\arraystretch{1.0}
\setlength{\tabcolsep}{5mm}
\scalebox{0.8}{
\begin{tabular}{lc}
\toprule
\textbf{Configuration} & \textbf{Value} \\
\midrule
    Graph encoder $f_g$ init. & $\text{GIN}_{\text{MoleculeSTM}}$ \\
    \# params $f_g$ & 1.8M \\
    LLM init. & Vicuna-v-1.3-7B \\
    \# params LLM & 6.9B \\
    Stage1 batch-size & 128 \\
    Stage2 batch-size & 128 \\
    Optimizer & AdamW \\
    Warm-up ratios & 0.03 \\
    Stage1 peak lr & 2e-3 \\
    Stage2 peak lr & 8e-5 \\
    Learning rate schedule & cosine decay \\
    Weight decay & 0. \\
    Stage1 train epochs & 5 \\
    Stage2 train epochs & 20-50 \\
    Numerical precision & bfloat16 \\
    Activation checkpointing & True \\
\bottomrule
\end{tabular}
}
\caption{\footnotesize{Training hyperparameters of InstructMol.}}
\label{training_detail}
\end{table}


\section{Evaluate Metrics}
\label{appendix:eval-metric}
\paragraph{Molecule Description Generation Metric.} 
Following \cite{MolT5}, NLP metrics such as BLEU~\cite{BLEU}, ROUGE~\cite{ROUGE} and METEOR~\cite{METEOR} are used to assess the proximity of generated descriptions to the truth of the ground. Specifically, these metrics are tested on the ChEBI-20 test dataset. In our experiments, we observed that after 50 epochs of finetuning on the training split, the metrics tend to converge, differing from previous approaches that often involved fine-tuning for over 100 epochs~\cite{MolT5, MoMu, MolFM}.

\paragraph{Molecule Generation Metric.}
In chemical reaction tasks, we view it as akin to a text-based molecule generation task. Initially, we employ RDKit to validate the chemical validity of the generated results, ensuring their ``validity". Subsequently, we gauge the sequential proximity between the generated sequence and the ground truth using NLP metrics such as BLEU, Exact Match scores, and Levenshtein distance. Additionally, we present performance based on molecule-specific metrics that assess molecular similarity, encompassing RDKit, MACCS~\cite{MACCS}, and Morgan~\cite{Morgan} fingerprints similarity. 

\begin{table*}[ht]
\centering
\footnotesize
\setlength{\tabcolsep}{0.1mm}{
\scalebox{0.95}{
\begin{tabular}{p{3cm}p{11.5cm}}
\toprule
\textbf{\textsc{Task}} & \textbf{\textsc{Instruction}} \\ \hline
Alignment Pretrain  & \makecell[l]{Instruction: \textit{Provide a brief overview of this molecule.}\\ \textit{$\mathbin\Vert\ [$Optional: The compound SELFIES sequence is: } \texttt{SELFIES}$]$ \\ Output: \textit{The molecule is a non-proteinogenic alpha-amino acid that is ...} } \\ 
\hline
%
\makecell[l]{Property Prediction \\(Regression)}  &  \makecell[l]{Instruction: \textit{Could you give me the LUMO energy value of this molecule?}\\ \textit{$\mathbin\Vert\ [$Optional: The compound SELFIES sequence is: } \texttt{SELFIES}$]$ \\ Output: \textit{0.0576} } \\
\hline
% 
\makecell[l]{Property Prediction \\(Classification)} & \makecell[l]{Instruction: \textit{Evaluate whether the given molecule is able to enter the blood-brain barrier.}\\ \textit{$\mathbin\Vert\ [$Optional: The compound SELFIES sequence is: } \texttt{SELFIES}$]$ \\ Output: \textit{Yes} } \\
\hline
% 
Molecule Description Generation & \makecell[l]{Instruction: \textit{Could you give me a brief overview of this molecule?}\\ \textit{$\mathbin\Vert\ [$Optional: The compound SELFIES sequence is: } \texttt{SELFIES}$]$ \\ Output:\textit{The molecule is a fatty acid ester obtained by ...}  } \\
\hline
% 
Forward Prediction & \makecell[l]{Instruction: \textit{Based on the given reactants and reagents, suggest a possible product.}\\ $\mathbin\Vert\ $\texttt{<REACTANT A>.<REACTANT B>...<REAGENT A>.<REAGENT B>...} \\ Output: \texttt{SELFIES} of product } \\
\hline
%
Retrosynthesis &  \makecell[l]{Instruction: \textit{Please suggest potential reactants used in the synthesis of the provided product.}\\ $\mathbin\Vert\ $\texttt{SELFIES} of product \\ Output: \texttt{<REACTANT A>.<REACTANT B>...<REAGENT A>.<REAGENT B>...}  } \\
\hline
%
Reagent Prediction  &  \makecell[l]{Instruction: \textit{Can you provide potential reagents for the following chemical reaction?}\\ $\mathbin\Vert\ $ \texttt{<REACTANT A>.<REACTANT B>...<REAGENT A>.<REAGENT B>... >> <PRODUCTs>}  \\ Output: \texttt{SELFIES} of reagent }  \\
\bottomrule
\end{tabular}
}}
\caption{
    Examples of instruction samples for each task. $\mathbin\Vert$ means concatenate along the token length dimension.
}
\label{tab:appendix-dataset}
\end{table*}


% classification prompt
\vskip 2in
\begin{table*}[h!]\centering
\begin{minipage}{\textwidth}\vspace{0mm}    
\centering
\begin{tcolorbox} 
    \centering
    \small
\begin{tabular}{p{1.0\textwidth}}

\VarSty{messages} = [
            \{\var{"role":"system", "content":} \var{f"""}You're acting as a molecule property prediction assistant. You'll be given SMILES of molecules and you need to make binary classification with a return result only in ``True" or ``False". \\
            \\ 
\textbf{The background of the dataset and task is shown below:} \\
The Blood-brain barrier penetration (BBBP) dataset comes from a recent study on the modeling and prediction of barrier permeability. As a membrane separating circulating blood and brain extracellular fluid, the blood-brain barrier blocks most drugs, hormones, and neurotransmitters. Thus penetration of the barrier forms a long-standing issue in the development of drugs targeting the central nervous system.   \\
\\
We provide several examples for this binary classification task: \\
\#\#\# \\
Instruction: Predict whether the given compound has barrier permeability. Return True or False.\\ 
SMILES: CCC(=O)C(CC(C)N(C)C)(c1ccccc1)c2ccccc2 \\
Output: True \\
\#\#\# \\
\\
\#\#\# \\
Instruction: Predict whether the provided compound exhibits barrier permeability. Return True or False.\\ 
SMILES: c1cc2c(cc(CC3=CNC(=NC3=O)NCCSCc3oc(cc3)CN(C)C)cc2)cc1 \\
Output: False \\
\#\#\# \\
... \\
\\

Given the following instructions and SMILES, return your prediction result: \\
Instruction: Predict whether the provided compound exhibits barrier permeability. Return True or False. \\
SMILES: \var{TARGET SMILES} \\


\var{"""}\}\\
]
\\
\end{tabular}
\end{tcolorbox}
\vspace{-2mm}
\caption{An illustration of the few-shot in-context-learning prompt construction process for Llama~\cite{Llama, Llama2} / Vicuna~\cite{vicuna} models in property prediction tasks.}
\label{tab:appendix-ICL-prompt}
\end{minipage}
\end{table*}

\clearpage
\section{Qualitative Analysis}
Several examples of different task results are shown in Figure~\ref{fig:qualitative_examples}. Figure~\ref{fig:qualitative_examples} (a-c) demonstrate the remarkable proficiency of InstructMol in accurately generating compounds related to chemical reaction prediction tasks. In Figure~\ref{fig:qualitative_examples} (d), InstructMol produces captions that closely match the ground truth, providing an accurate description of the \textbf{family} (i.e. \textit{``a member of the class of indole-3-acetic acids"}), \textbf{structure} (i.e. \textit{``the hydrogen at position 5 has been replaced by a carboxy group"}) and \textbf{biological activity} (i.e. \textit{``It has a role as a bacterial metabolite."}).

\begin{figure*}
    \vskip -0.2in
    \centering
    \includegraphics[width=0.98\linewidth,]{fig/examples.pdf}
    \caption{\footnotesize Comparison of chemical reaction and molecule description generation tasks results. \textbf{(a-c)} demonstrate the performance relative to baselines~\cite{Mol-Instructions, Text+ChemT5}, highlighting InstructMol's precise generation of reaction-related compounds. \textbf{(d)} reveals InstructMol's caption aligning closely with the ground truth. The colored text represents the exact match between the output of InstructMol and the ground truth.}
    \label{fig:qualitative_examples}
\end{figure*}


\newpage
\section{More Downstream Examples}
\label{appendix:more-examples}

\subsection{More Results of Molecule Description Generation}
\begin{figure*}[!ht]
    \centering
    \includegraphics[width=1.05\linewidth]{fig//supp/molcap.pdf}
    \caption{More examples of molecule description generation task on ChEBI-20~\cite{Text2Mol} test set. We include Mol-Instruction~\cite{Mol-Instructions} as the baseline. CID: PubChem Compound Identification, a non-zero integer PubChem accession identifier for a unique chemical structure. }
    \label{fig:appendix-molcap}
\end{figure*}

\clearpage
\subsection{More Results of Forward Reaction Prediction}
\begin{figure*}[!ht]
    \centering
    \includegraphics[width=1\linewidth]{fig//supp/forward.pdf}
    \caption{More examples of forward reaction prediction task. We include Mol-Instruction~\cite{Mol-Instructions} and Multitask-Text-and-Chemistry-T5~\cite{Text+ChemT5} as baselines.}
    \label{fig:appendix-forward}
\end{figure*}

\clearpage
\subsection{More Results of Reagent Prediction}
\begin{figure*}[!ht]
    \centering
    \includegraphics[width=1\linewidth]{fig//supp/reagent.pdf}
    \caption{More examples of the reagent prediction task. We include Mol-Instruction~\cite{Mol-Instructions} as the baseline.}
    \label{fig:appendix-reagent}
\end{figure*}

\clearpage
\subsection{More Results of Retrosynthesis Prediction}
\begin{figure*}[!ht]
    \centering
    \includegraphics[width=1\linewidth]{fig//supp/retro.pdf}
    \caption{More examples of the retrosynthesis prediction task. We include Mol-Instruction~\cite{Mol-Instructions} and Multitask-Text-and-Chemistry-T5~\cite{Text+ChemT5} as baselines.}
    \label{fig:appendix-retro}
\end{figure*}

\clearpage
\subsection{Difficult Cases}
We showcase cases with misalignment to the ground truth, along with RDKit fingerprint similarity results in Fig.~\ref{fig:appendix-failure}. The complexity of chemical reaction compounds makes the task more challenging. In addressing this limitation, our future approach involves concatenating graph tokens from multiple molecules involved in the same reaction with text tokens to simplify the complexity of the input sequence. Moreover, we are considering employing separate tokenization and embedding for distinct modalities to ensure the semantic accuracy of the tokenized results.

\begin{figure*}[!ht]
    \centering
    \includegraphics[width=1\linewidth]{fig//supp/failure.pdf}
    \caption{We present several cases with a certain degree of misalignment compared to the ground truth, accompanied by RDKit fingerprint similarity results relative to the ground truth. Due to the heightened complexity of compounds involved in chemical reactions, the difficulty of the task increases, leading to the poor performance of Mol-Instructions~\cite{Mol-Instructions}.}
    \label{fig:appendix-failure}
\end{figure*}


\section{Comparison with Current Agents}
\label{appendix:Comparison_with_agents}
LLMs face a major limitation in performing basic mathematical and chemical operations, which makes handling hallucinations challenging. However, their self-supervised pre-training on diverse knowledge equips them with a strong understanding and reasoning abilities that can be directly applied to new domains. Presenting LLMs as automated assistants offers a programming-free interface for non-experts to leverage their existing capabilities. Agent/assistant paradigms enable the optimal utilization of LLMs' knowledge without the need for specialized model development. For instance, ChemCrow \cite{ChemCrow} is an agent system based on GPT-4 that integrates various chemical tools for solving diverse tasks. We conducted a comparison of three downstream tasks between InstructMol and ChemCrow, and the results are presented in Table \ref{tab:LLMAgents}.

During testing, we observed that ChemCrow's performance is heavily reliant on prompt construction, resulting in unstable output results. For instance, in retrosynthesis planning experiments, we found that agents often misidentify the user's query product as controlled chemistry and refuse to provide an answer. Similarly, in the property prediction task, GPT-4 itself lacks specific knowledge about compounds and thus heavily relies on internet searches. The quality of the prompt constructed by the user significantly influences the quality of the response.

\begin{table}[h]
\centering
\renewcommand\arraystretch{1.0} 
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{lccc}
\hline
\textbf{Task} & \textbf{Ground Truth} & \textbf{ChemCrow} & \textbf{InstructMol}\\
\hline
\rowcolor[RGB]{234, 238, 234}
\multicolumn{4}{l}{\textit{Property Prediction}} \\
\makecell[l]{Determine whether (CID:219214)\\ can suppress HIV.} & "Active" & \makecell[l]{WebSearch$\rightarrow$ \\ No information} & $\checkmark$ \\ \hline
\rowcolor[RGB]{234, 238, 234}
\multicolumn{4}{l}{\textit{Forward Reaction Prediction}} \\
\scriptsize{CCC(=O)Cl $+$ OC1=CC=CC(F)=C1}\\ \scriptsize{$+$ ClCCl $+$C2=CC=NC=C2 $\rightarrow ?$}  & \scriptsize{CCC(=O)OC1=CC=CC(F)=C1} & $\checkmark$  & $\checkmark$  \\ \hline

\rowcolor[RGB]{234, 238, 234}
\multicolumn{4}{l}{\textit{Retrosynthesis Prediction}} \\ 
$?\rightarrow$ \scriptsize{C(CCNC(=O)CCCCBr)CCO} & \scriptsize{NCCCCCO.O=C(O)CCCCCBr} & \makecell[l]{"Similar to controlled \\chemistry, reject to answer"} & $\checkmark$  \\
\bottomrule
\end{tabular}
}
\caption{\footnotesize{The performance of InstructMol and ChemCrow was evaluated through a comparison of three downstream tasks: Property Prediction, Forward Reaction Prediction, and Retrosynthesis. The $\checkmark$ denotes that the predictions match with the ground truths.}}
\label{tab:LLMAgents}
\end{table}

Therefore, we believe that domain-specific LLMs should be augmented with dedicated external tools. This augmentation would enable LLMs to function as planners, comprehend and decompose tasks, invoke downstream interfaces, and effectively process feedback. In our future work, we intend to create a new dataset for instruction-following tool usage and enhance InstructMol with a variety of external tools. By leveraging state-of-the-art models and maximizing LLM's reasoning and planning capabilities, we aim to further enhance its performance.
